Decoupling Collision Avoidance in and for Optimal Control using Least-Squares Support Vector Machines

This paper details an approach to linearise differentiable but non-convex collision avoidance constraints tailored to convex shapes. It revisits introducing differential collision avoidance constraints for convex objects into an optimal control problem (OCP) using the separating hyperplane theorem. By framing this theorem as a classification problem, the hyperplanes are eliminated as optimisation variables from the OCP. This effectively transforms non-convex constraints into linear constraints. A bi-level algorithm computes the hyperplanes between the iterations of an optimisation solver and subsequently embeds them as parameters into the OCP. Experiments demonstrate the approach's favourable scalability towards cluttered environments and its applicability to various motion planning approaches. It decreases trajectory computation times between 50\% and 90\% compared to a state-of-the-art approach that directly includes the hyperplanes as variables in the optimal control problem.

==> Sections/validation.tex <==
% !TeX root = ../root.tex
\label{sec:validation}

% Cost per iter mumps: 3.14 ms full, 1.82 ms decoupled best
% \setlength{\extrarowheight}{5pt}
% \setlength{\tabcolsep}{1pt}

% Note that this effect is only shown for a simple motion planning problem. For more complex examples (larger amount of obstacles, more complex dynamics, etc.), the aforementioned effects such as for example the increase in iterations with an decrease in the angular trust-region boundary will be more pronounced. {\color{red} Add example data for more obstacles for angle.}



{\color{red} Run validation over many environments as well}

\begin{itemize}
    \item Object picking in industrial environment
    \item 2D-spline based motion planning (3D with drone?)
    \item Comparison with OMGtools as coupled approach
    \item Explain why hyperplane classification is relevant to this example
    \item Validate compared to coupled approach + {\color{red} Different approach ?} in terms of:
    \begin{itemize}
        \item Computation time (remove part of non-convexity)
        \item Execution time (avoid certain local minima + possible added conservativeness)
        \item Succes rate over various environments / tasks?
    \end{itemize}
    \item 
\end{itemize}
\paragraph{Experiment Set-up}
Both approaches are used to compute a trajectory through a pseudo-randomly generated environment with two to six obstacles. For each environment, trajectories between {\color{red} eight} different start and end configurations are computed, {\color{red} divided such that the whole environment is traversed}. A set of {\color{red} ... } environments is generated per fixed number of obstacles, leading to a validation set of {\color{red}...} trajectories. The OCP is solved using IPOPT with a maximum of 100 iterations, using the linear solver MA27~\cite{hsl}. A horizon of 10 is chosen, the radius of the vehicle is 0.5 and 
The hyperplane parameters are initialised with zeros and the initial guess for the trajectory is a straight line between the start and end configuration. The OCP is solved with a horizon of 20, a maximum velocity of 1 m/s and time-optimal objective function. The experiments are conducted on a portable computer with an Intel® Core™ i7-10810U processor with twelve cores at 1.10GHz and 31.1 GB RAM.

{\color{red} Add parameters from filters for these experiments.}

\paragraph{Results}
Table~\ref{tab:results_splines} summarises the results of the experiments. The wall time reports the total time needed to solve the OCP, the time per iteration is described by the second row. LS wall time reports the additional overhead introduced by solving Eq.~\ref{eq:lssvm} or Eq.~\ref{eq:qpsvm} without slacks $e_{k}$. The success rate is the percentage of trajectories that are collision-free, the optimality is relative to the best optimal cost between two approaches{\color{red} relative to high horizon full OCP without splines?} and the number of iterations is relative to the lowest number of iterations between both approaches, compared per trajectory. The last two rows indicate the average amount of times both Eq.~\ref{eq:qpsvm} and~\ref{eq:lssvm} are solved to find one trajectory.

{\color{red} Add results of experiments}
\begin{itemize}
    \item Wall time: median reduction of 53.75\% for SVM approach
    \item Success rate: decrease of 2\% for SVM approach
    \item Conservativeness: median increase of 0.7\% for SVM approach
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{chapters/hyperplanes/Images/splines_N10_2obsts.png}
    \caption{Comparison between the coupled and decoupled approach for the spline-based motion planning problem. The left plot shows the wall time needed to solve the OCP, the right plot shows the reduction of the cost per iteration. The red stars indicate where no feasible solution to a problem could be found be one or both methods.} 
    \label{fig:spline_results_2obst}
\end{figure}

\renewcommand{\arraystretch}{1.0}
% \begin{sidewaystable}
% \centering
\begin{table}[H]
    \caption{\small{Comparison between both approaches for the spline-based motion planning problem. }}
    \centering
    \tablefontsize
    \begin{tabularx}{\linewidth}{@{} YYYYYYYY @{}}
        \toprule
        \multirow{2}{*}{\textbf{Characteristic}} & \multirow{2}{*}{\textbf{Approach}} & \multicolumn{5}{c}{\textbf{\# obstacles}} \\
        \cmidrule[0.1pt]{3-7}
        & & 2 & 3 & 4 & 5 & 6\\
        % \multicolumn{2}{c}{\textbf{\# obstacles}} & 2 & 3 & 4 & 5 & 6\\
        % \midrule[0.05pt]
        \midrule[0.1pt] \midrule[0.1pt]
        \multirow{2}{*}{\textbf{$t_{\text{wall}}$ (ms)}} & SVM & \textbf{27.73} & 234.06 & ... & ... & ... \\
        & Coupl. & 59.97 & 472.90 & ... & ... & ... \\
        \cmidrule[0.05pt]{2-7}
        \multirow{2}{*}{\textbf{$t_{\text{wall}}$ / iter (ms)}} & SVM & \textbf{1.66} & 10.83 & ... & ... & ... \\
        & Coupl. & 2.51 & 16.31 & ... & ... & ... \\
        \cmidrule[0.05pt]{2-7}
        \multirow{2}{*}{\textbf{$t_{\text{wall}}$ LS (ms)}} & SVM & 0.10 & 1121 & ... & ... & ... \\
        & Coupl. & - & - & - & - & - \\
        \cmidrule[0.05pt]{2-7}
        \multirow{2}{*}{\textbf{Success (\%)}} & SVM & 93 & 78 & ... & ... & ... \\
        & Coupl. & \textbf{95} & 84 & ... & ... & ... \\
        \cmidrule[0.05pt]{2-7}
        \multirow{2}{*}{\textbf{Optimality (\%)}} & SVM & 1.01 & 1.02 & ... & ... & ... \\
        & Coupl. & \textbf{1.0} & 1.0 & ... & ... & ... \\
        \cmidrule[0.05pt]{2-7}
        \multirow{2}{*}{\textbf{Iterations (\%)}} & SVM & \textbf{0.76} & 0.77 & ... & ... & ... \\
        & Coupl. & 1.0 & 1.0 & ... & ... & ... \\
        \cmidrule[0.05pt]{2-7}
        \multirow{2}{*}{\textbf{\# LS (-)}} & SVM & 9.63 & 24.1 & ... & ... & ... \\
        & Coupl. & - & - & - & - & - \\
        \cmidrule[0.05pt]{2-7}
        \multirow{2}{*}{\textbf{\# QP (-)}} & SVM & 23.88 & 45.16 & ... & ... & ... \\
        & Coupl. & - & - & - & - & - \\
        \bottomrule
    % \multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
    \end{tabularx}
    \label{tab:results_splines}
\end{table}
% \end{sidewaystable}

\subsection{Object Picking with 6-DOF Robotic Manipulator}
One capsule, one environment and 20 trajectories
\renewcommand{\arraystretch}{1.5}
\begin{sidewaystable}
\centering
\begin{table}[H]
    \caption{\small{Comparison between both approaches for the robotic arm motion planning.}}
    \centering
    \tablefontsize
    \begin{tabularx}{\linewidth}{@{} YYYYYYYYY @{}}
        \toprule
        \multirow{2}{*}{\textbf{Characteristic}} & \multicolumn{8}{c}{\textbf{Approach}} \\
        \cmidrule[0.1pt]{2-9}
        & Coupl. & Best & (1) & (2) & (3) & (4) & (5) & (6) \\
        % \multicolumn{2}{c}{\textbf{\# obstacles}} & 2 & 3 & 4 & 5 & 6\\
        % \midrule[0.05pt]
        \midrule[0.1pt] \midrule[0.1pt]
        \textbf{$t_{\text{wall}}$(ms)} & ... & ... & ... & ... & ... & ... & ... & ...\\
        \textbf{$t_{\text{wall}}$ / iter (ms)} & ... & ... & ... & ... & ... & ... & ... & ... \\
        \textbf{$t_{\text{wall}}$ LS (ms)} & ... & ... & ... & ... & ... & ... & ... & ... \\
        \textbf{Success rate (\%)} & ... & ... & ... & ... & ... & ... & ... & ... \\
        \textbf{Optimality (\%)} & ... & ... & ... & ... & ... & ... & ... & ... \\
        \textbf{Iterations (\%)} & ... & ... & ... & ... & ... & ... & ... & ... \\
        \textbf{\# LS (-)} & ... & ... & ... & ... & ... & ... & ... & ... \\
        \textbf{\# QP (-)} & ... & ... & ... & ... & ... & ... & ... & ... \\
        \bottomrule
    % \multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
    \end{tabularx}
    \label{tab:results_svm_arm}
\end{table}
\end{sidewaystable}

\paragraph{Results}
Table~\ref{tab:results_svm_arm} summarises the results of the experiments. The wall time reports the total time needed to solve the OCP, the time per iteration is described by the second row. LS wall time reports the additional overhead introduced by solving Eq.~\ref{eq:lssvm} or Eq.~\ref{eq:qpsvm} without slacks {\color{red} Need to explain this in bi-level step}. The success rate is the percentage of trajectories that are collision-free, the optimality is relative to the best optimal cost between two approaches {\color{red} relative to high horizon full OCP without splines?} and the number of iterations is relative to the lowest number of iterations between both approaches, compared per trajectory. The last two rows indicate the average amount of times both Eq.~\ref{eq:lssvm} and~\ref{eq:qpsvm} are solved to find one trajectory.

{\color{red} Vary environment and run experiments for them as well --> how to generate feasible initial poses ?}

\subsection{Discussion}
However, the proposed approach is not limited to these two cases and is applicable to any path planning, OCP or MPC algorithm involving collision avoidance with a convexly modelled environment.

